Jet energy scale determination in the D0 experiment

The calibration of jet energy measured in the \DZero detector is presented, based on ppbar collisions at a center-of-mass energy of 1.96 TeV at the Fermilab Tevatron collider. Jet energies are measured using a sampling calorimeter composed of uranium and liquid argon as the passive and active media, respectively. This paper describes the energy calibration of jets performed with photon+jet, Z+jet and dijet{} events, with jet transverse momentum pT > 6 GeV and pseudorapidity range |eta| < 3.6. The corrections are measured separately for data and simulation, achieving a precision of 1.4%-1.8% for jets in the central part of the calorimeter and up to 3.5% for the jets with pseudorapidity |eta| = 3.0. Specific corrections are extracted to enhance the description of jet energy in simulation and in particular of the effects due to the flavor of the parton originating the jet, correcting biases up to 3%-4% in jets with low pT originating from gluons and up to 6%-8% in jets from b quarks.

==> listofchanges.tex <==
\section*{Editorial notes}
% \label{sec:EditorialNotes}
% 
% \subsection*{To do list in this version of the NIM paper}
% \label{ssec:ToDos}
% 
% \begin{itemize}
% 	\item write Introduction chapter
% 	\item write Detector/Calorimeter chapter
% 	\item write Data Quality Requirement 
% 	\item write Flavor Dependent Corrections chapter
% 	\item write QCD Specific Correction chapter
% 	\item write JSSR chapter
% 	\item rewrite High Energy Extrapolation chapter
% 	\item rewrite Showering chapter
% 	\item rewrite Correlation chapter
% \end{itemize}

\subsection*{List of changes}
\label{ssec:Changes}

The paper is available in the \DZero{} documents CVS repository as \texttt{jes\_nim}.\\
Dmitry Bandurin, Bob Hirosky, Bob Kehoe and Gianluca Petrillo have committing privileges.


\subsubsection*{\texttt{v01-03-00}}

First draft for review by the Editorial Board


\subsubsection*{\texttt{v01-03-01}}
\begin{itemize}
	\item lots of minor fixes in the notation (also in plots)
\end{itemize}

\subsubsection*{\texttt{v01-03-02}}
\begin{itemize}
	\item fixes in the notation of the closure plots
\end{itemize}

\subsubsection*{\texttt{v01-03-03}}
\begin{itemize}
	\item fixes in the notation of the single particle response closure plots
\end{itemize}

\subsubsection*{\texttt{v01-03-04}}
\begin{itemize}
	\item erratum in \cref{feta_gj_procedure}: the definition of \Feta[\photonjet] has pure \photonjet MPF
	\item reordering sections: sections about summary plots and JES closure tests moved before the single particle response tuning (\cref{sec:fdc})
	\item SSR (\cref{sec:jssr}) expanded to explain how we use the result in \DZero
\end{itemize}

\subsubsection*{\texttt{v01-03-05}}
\begin{itemize}
	\item final version of the plot in \cref{fig:qg_frac_zj}
	\item a few style modification of figures
	\item implemented EB comments from Bob Hirosky, Christoph Royon, Bjoern Penning
\end{itemize}

\subsubsection*{\texttt{v01-03-06}}
\begin{itemize}
	\item implementing further comments from Bob Hirosky
\end{itemize}

\subsubsection*{\texttt{v01-04-00}}
\begin{itemize}
	\item version entering style review on August \nth{16}, 2013 (same as 1.3.6)
\end{itemize}


\subsubsection*{\texttt{v02-00-00}}
\begin{itemize}
	\item all comments from style review integrated
	\item version for collaboration review on September \nth{18}, 2013
\end{itemize}


\subsubsection*{\texttt{v02-01-00}}
\begin{itemize}
	\item comments from Rick Van Kooten integrated
\end{itemize}


\subsubsection*{\texttt{v02-02-00}}
\begin{itemize}
	\item comments from Leo Bellantoni and Dmitri Denisov integrated
\end{itemize}


\subsubsection*{\texttt{v02-03-00}}
\begin{itemize}
	\item all pending comments integrated
	\item sign off version
\end{itemize}

\subsubsection*{\texttt{v02-03-02}}
\begin{itemize}
	\item comments from Dmitry, Gregorio and Bob integrated
\end{itemize}

\subsubsection*{\texttt{v02-04-00}}
\begin{itemize}
	\item comments from Rick and George integrated
	\item final revision version
\end{itemize}


\subsubsection*{To be changed}
\begin{itemize}
% 	\item check/fix the order/numbering of \cref{fig:Summary_CorrVsEta_JCCB_DATA,fig:Summary_CorrVsEta_JCCA_DATA,fig:Summary_ErrVsEta_JCCB_DATA}
% 	\item checked is "accepted" references have become published
\end{itemize}


% \subsubsection*{(future \texttt{v01-03-06})}
% \begin{itemize}
% 	\item fixes in the notation of the closure plots
% \end{itemize}
% 

